Dataset Dynamics via Gradient Flows in Probability Space

Various machine learning tasks, from generative modeling to domain adaptation, revolve around the concept of dataset transformation and manipulation. While various methods exist for transforming unlabeled datasets, principled methods to do so for labeled (e.g., classification) datasets are missing. In this work, we propose a novel framework for dataset transformation, which we cast as optimization over data-generating joint probability distributions. We approach this class of problems through Wasserstein gradient flows in probability space, and derive practical and efficient particle-based methods for a flexible but well-behaved class of objective functions. Through various experiments, we show that this framework can be used to impose constraints on classification datasets, adapt them for transfer learning, or to re-purpose fixed or black-box models to classify -- with high accuracy -- previously unseen datasets.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%						USEFUL PREAMBLES FOR LATEX FILES                       %
%																			   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% THIS FILE IS CUSTOMIZABLE, RELIES ON THE FOLLOWING BOOLEAN VARIABLES:

% NOTE: \providebool Defines boolean flag unless already defined (from package etoolbox)

\usepackage{etoolbox}
\providebool{loadgeometry} % will default to false
\providebool{altermargins} % will default to false
\providebool{usebiblatex}  % will default to false


\setbool{loadgeometry}{false}
%\setbool{usebiblatex}{false}

% \ifcsundef{conference}{
% 	\providebool{conference} % Whether or not this is a conference paper.
% 	\setbool{conference}{false}
% 	\typeout{Variable conference undefined. Initializing.}
% }{}
% \ifcsundef{biblatex}{
% 	\providebool{biblatex}   % Whether to use biblatex instead of natbib
% 	\setbool{biblatex}{true}
% 	\typeout{Variable biblatex undefined. Initializing.}
% }{}



% #################    FONTS   #################
%\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc} % use 8-bit T1 fonts
\usepackage{tgtermes}

% NOTE: MUST INSTALL SEPARATELY
% \usepackage[subscriptcorrection,
%            amssymbols,
%            mtpbb,
%            mtpcal,
%            nofontinfo  % suppresses all warnings
%           ]{mtpro2}
% NOTE: MUST UNCOMMENT IF NOT USING MTPRO2
\usepackage{amssymb}
\newcommand{\mathbold}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}

\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \renewcommand*\ttdefault{lmvtt}
\usepackage[ttdefault=true]{AnonymousPro}

% #################    MATH   #################
\usepackage{amsmath}
\usepackage{amsmath,amsthm, mathtools}
\usepackage{amscd}
\usepackage{bbm}
% \usepackage{bm}          % Bold math symbols
\usepackage{commath}      % Differentials, etc
\usepackage{dsfont}       % For \mathds
\usepackage{upgreek}      % For \upalpha etc
\usepackage{stmaryrd}     % For nice double bracket [[ ]] 
\usepackage{siunitx}      % Scientific notation
\usepackage{xspace}
\usepackage{float}        % For H in tables/figs


% #################    SPACING AND TEXT   #################

\ifbool{loadgeometry}{
	\ifbool{altermargins}{
		% For free-form papers:
		\usepackage[
		  paper  = letterpaper,
		  left   = 1.25in,
		  right  = 1.25in,
		  top    = 1.0in,
		  bottom = 1.0in,
		  ]{geometry}
	}{
		\usepackage{geometry} 	% For conference/journal papers, don't mess with margins
	}
}

% \usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xspace}
\usepackage{xparse}% http://ctan.org/pkg/xparse
\usepackage{csquotes} % To silence warning by biblatex


% #################    EDITING    #################

%%% Remove these for conferences, etc
%\usepackage{layouts} % To display of various elements of a document’s  layout. 
%\usepackage{lineno}
%\renewcommand\linenumberfont{\normalfont
%                              \footnotesize
%                              \sffamily
%                              \color{SkyBlue}}

% \usepackage{ragged2e}
% \DeclareRobustCommand{\sidenote}[1]{\marginpar{
%                                     \RaggedRight
%                                     \textcolor{Plum}{\textsf{#1}}}}

% \newcommand{\parnum}{\bfseries\P\arabic{parcount}}
% \newcounter{parcount}
% \newcommand\p{%
%     \stepcounter{parcount}%
%     \leavevmode\marginpar[\hfill\parnum]{\parnum}%
% }
% \DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}
% \ifbool{altermargins}{
% 	\setlength{\marginparwidth}{1.25in}
% }{}

% #################    COLOR    #################

\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% #################    COUNTERS    #################

\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% #################  FIGURES AND TABLES   #################

\usepackage[pdftex]{graphicx}
\usepackage[labelfont=bf]{caption}
%\usepackage[hypcap=true]{caption}
\usepackage[format=hang]{subcaption}
\usepackage{booktabs, array}
\usepackage{wrapfig}
\usepackage{graphbox} % additional options for includegraphics, e.g. align

% #################    ALGORITHMS    #################

\usepackage[algoruled]{algorithm2e}
\setlength{\interspacetitleruled}{8pt}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\small}


% #################   ACRONYMS  #################

\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}

% #################   BIB AND LINKS  #################

\usepackage[colorlinks,linktoc=all]{hyperref} % should be one of the last packages to load always
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\usepackage[nameinlink]{cleveref} % must always be loaded after hyperref
\creflabelformat{equation}{#2\textup{#1}#3}  % <- remove parenthesis from eqs
\crefname{section}{§}{§§}
\Crefname{section}{§}{§§}

% #################  CODE SNYPPETS  #################

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% #################  BIBLIOGRAPHY #################

\ifbool{usebiblatex}{
	\usepackage[
	    backend=biber,
		citestyle=numeric-comp,
	    defernumbers=true,       % continuous numbering across bibliography sections
		giveninits=true,         % abbreviate first name
		natbib=true,
		isbn=false,
    	maxnames=2, % max number of names to display before switching to et al in main text
    	%maxbibnames=8, % max number of names to display before switching to et al in bibliogrtaphuy		
		%sorting=none,
		eprint=true,
		url=false,
		doi=false,
	]{biblatex}
	\setlength\bibitemsep{0.2\baselineskip}
}{
	\usepackage{natbib}
}



% #################   USEFUL COMMANDS  #################

\newcommand{\pp}{\textcolor{Plum}{\P\,}}
\newcommand{\q}[1]{\red{{\sf Q | #1}}}
\newcommand{\draftdisclaimer}{\begin{center}\begin{framed} DRAFT: DO
NOT CITE OR DISTRIBUTE \end{framed}\end{center}}



% #################   TODOS  #################


% 
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%


% % Preamble with lots of Macros for Optimization Problems
%
%
% %% Language and font encodings
% \usepackage[english]{babel}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%
%
% \usepackage[dvipsnames,usenames]{color}
% \definecolor{NavyBlue}{cmyk}{0.94,0.54,0,0}
% \definecolor{DarkBlue}{rgb}{0,0.2,0.6}
%
% %\usepackage[colorlinks=true, allcolors=blue]{hyperref}     % hyperlinks
% \usepackage[colorlinks=true, linkcolor=BrickRed,citecolor=DarkBlue,urlcolor=DarkBlue,bookmarks=false]{hyperref}
% %\usepackage[hidelinks]{hyperref}. %% Liks are live but black
%
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
%
% \usepackage{enumerate}
% \usepackage{enumitem}   % For easy chaning numbers to letters
%
% %% Sets page size and margins
% \usepackage[pdftex]{graphicx}
% %\usepackage[a4paper,top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}
%
% %% Useful packages
% %\usepackage{bbm}          % bold math symbols
%
% %% AMS stuff
% \usepackage{amssymb,amsmath,amsthm, mathtools}
% \usepackage{amscd}
%
%
% %\usepackage{subfigure}
% \usepackage{caption, subcaption}% http://ctan.org/pkg/{caption,subcaption}
% \usepackage{float} % To use the H option in \figure
%
%
% \usepackage{fancyhdr}
% \usepackage{titlesec}
%
% %% For algorithms
% \usepackage{algorithm}
% \usepackage{algorithmic}
%
%


==> preamble_pkgs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%						USEFUL PREAMBLES FOR LATEX FILES                       %
%																			   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% THIS FILE IS CUSTOMIZABLE, RELIES ON THE FOLLOWING BOOLEAN VARIABLES:

% NOTE: \providebool Defines boolean flag unless already defined (from package etoolbox)

\RequirePackage{etoolbox}
\providebool{loadgeometry} % will default to false
\providebool{loadhyperref} % will default to false
\providebool{altermargins} % will default to false
\providebool{usebiblatex}  % will default to false


% \setbool{loadgeometry}{false}
% \setbool{loadhyperref}{false}
% \setbool{usebiblatex}{true}

% \ifcsundef{conference}{
% 	\providebool{conference} % Whether or not this is a conference paper.
% 	\setbool{conference}{false}
% 	\typeout{Variable conference undefined. Initializing.}
% }{}
% \ifcsundef{biblatex}{
% 	\providebool{biblatex}   % Whether to use biblatex instead of natbib
% 	\setbool{biblatex}{true}
% 	\typeout{Variable biblatex undefined. Initializing.}
% }{}

% #################    FONTS   #################
\usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}    % This might change some fonts, e.g, bold title in imsart style
\usepackage{tgtermes}

% NOTE: MUST INSTALL SEPARATELY
% \usepackage[subscriptcorrection,
%            amssymbols,
%            mtpbb,
%            mtpcal,
%            nofontinfo  % suppresses all warnings
%           ]{mtpro2}
% NOTE: MUST UNCOMMENT IF NOT USING MTPRO2
\usepackage{amssymb}

%\newcommand{\mathbold}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}

\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \renewcommand*\ttdefault{lmvtt}
\usepackage[ttdefault=true]{AnonymousPro}

% #################    MATH   #################
\usepackage{amsmath}
\usepackage{amsmath,amsthm, mathtools}
\usepackage{amscd}
\usepackage{bbm}
% \usepackage{bm}          % Bold math symbols
\usepackage{commath}      % Differentials, etc
\usepackage{dsfont}       % For \mathds
\usepackage{upgreek}      % For \upalpha etc
\usepackage{stmaryrd}     % For nice double bracket [[ ]] 
\usepackage{siunitx}      % Scientific notation
\usepackage{xspace}
\usepackage{float}        % For H in tables/figs


% #################    SPACING AND TEXT   #################

\ifbool{loadgeometry}{
	\ifbool{altermargins}{
		% For free-form papers:
		\usepackage[
		  paper  = letterpaper,
		  left   = 26.5mm,
		  right  = 26.5mm, %25mm
		  top    = 28mm,  %28mm
		  bottom = 28mm,  %30mm
		  ]{geometry}
	}{
		\usepackage{geometry} 	% For conference/journal papers, don't mess with margins
	}
}

% \usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
%\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xspace}
\usepackage{xparse}% http://ctan.org/pkg/xparse
\usepackage{csquotes} % To silence warning by biblatex

% To make \pargagraphs equally spaced as normal paragraphs
\usepackage{titlesec}
%\titlespacing*{\paragraph}{0pt}{0.25ex plus 1ex minus .2ex}{1em}
%\titlespacing*{\paragraph}{0pt}{0em plus 0.1em minus 0.2em}{1em}
%{1em plus 0.1em minus 0.2em}


% #################    EDITING    #################

\usepackage{lineno}
% \renewcommand\linenumberfont{\normalfont
%                              \footnotesize
%                              \sffamily
%                              \color{SkyBlue}}

\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}

\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}
\ifbool{altermargins}{
	\setlength{\marginparwidth}{1.25in}
}{}

% #################    COLOR    #################
\usepackage{color}
\usepackage[usenames,dvipsnames]{xcolor}
%\definecolor{shadecolor}{gray}{0.9}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}




% #################    COUNTERS    #################

\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% #################  FIGURES AND TABLES   #################

\usepackage[pdftex]{graphicx}
\usepackage[labelfont=bf]{caption}
%\usepackage[hypcap=true]{caption}
\usepackage[format=hang]{subcaption}
\usepackage{booktabs, array, multirow}
\usepackage{wrapfig}
\usepackage{graphbox} % additional options for includegraphics, e.g. align

% #################    ALGORITHMS    #################

\ifbool{loadalgorithm2e}{
    \usepackage[ruled,vlined]{algorithm2e}
    \setlength{\interspacetitleruled}{8pt}
    \newcommand\algocommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
    \SetCommentSty{algocommfont}
    \usepackage{fancyvrb}
    \fvset{fontsize=\small}
}

\usepackage{listings}

% #################   BIB AND LINKS  #################

\ifbool{loadhyperref}{
    \usepackage[colorlinks,linktoc=all]{hyperref}
    \hypersetup{citecolor=MidnightBlue}
    \hypersetup{linkcolor=MidnightBlue}
    \hypersetup{urlcolor=MidnightBlue}
}{}
\usepackage[nameinlink]{cleveref}
\creflabelformat{equation}{#2\textup{#1}#3}  % <- remove parenthesis from eqs
\crefname{section}{§}{§§}
\Crefname{section}{§}{§§}


% #################   ACRONYMS  #################

\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}

% #################  CODE SNYPPETS  #################

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% #################  BIBLIOGRAPHY #################

\ifbool{usebiblatex}{
	\usepackage[
	   % style=apa, % For AISTATS
	    style=authoryear,
	    backend=biber,
		citestyle=authoryear,
	    defernumbers=true,       % continuous numbering across bibliography sections
		giveninits=true,         % abbreviate first name
		doi=false,
		natbib=true,
		isbn=false,
    	maxnames=2, % max number of names to display before switching to et al in main text
		minnames=1, % If a list holds more than maxnames names, it is automatically truncated to minnames names + et al
    	maxbibnames=3, % similar to maxnames but affects only bibliography
    	minbibnames=3, % similar to minnames but affects only bibliography
		%sorting=none,
		eprint=true,
	    %uniquename=false,
		url=false,
	]{biblatex}
	%\setlength\bibitemsep{4\itemsep}
	\setlength\bibitemsep{0.3\baselineskip}
}{
	\usepackage{natbib}
}



% #################   USEFUL COMMANDS  #################

\newcommand{\pp}{\textcolor{Plum}{\P\,}}
\newcommand{\q}[1]{\red{{\sf Q | #1}}}
\newcommand{\draftdisclaimer}{\begin{center}\begin{framed} DRAFT: DO
NOT CITE OR DISTRIBUTE \end{framed}\end{center}}



% #################   TODOS  #################


% 
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%


% % Preamble with lots of Macros for Optimization Problems
%
%
% %% Language and font encodings
% \usepackage[english]{babel}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%
%
% \usepackage[dvipsnames,usenames]{color}
% \definecolor{NavyBlue}{cmyk}{0.94,0.54,0,0}
% \definecolor{DarkBlue}{rgb}{0,0.2,0.6}
%
% %\usepackage[colorlinks=true, allcolors=blue]{hyperref}     % hyperlinks
% \usepackage[colorlinks=true, linkcolor=BrickRed,citecolor=DarkBlue,urlcolor=DarkBlue,bookmarks=false]{hyperref}
% %\usepackage[hidelinks]{hyperref}. %% Liks are live but black
%
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
%
% \usepackage{enumerate}
% \usepackage{enumitem}   % For easy chaning numbers to letters
%
% %% Sets page size and margins
% \usepackage[pdftex]{graphicx}
% %\usepackage[a4paper,top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}
%
% %% Useful packages
% %\usepackage{bbm}          % bold math symbols
%
% %% AMS stuff
% \usepackage{amssymb,amsmath,amsthm, mathtools}
% \usepackage{amscd}
%
%
% %\usepackage{subfigure}
% \usepackage{caption, subcaption}% http://ctan.org/pkg/{caption,subcaption}
% \usepackage{float} % To use the H option in \figure
%
%
% \usepackage{fancyhdr}
% \usepackage{titlesec}

% %% For algorithms
% \usepackage{algorithm}
% \usepackage{algorithmic}
